A Computationally Efficient Learning-Based Model Predictive Control for Multirotors under Aerodynamic Disturbances

Neglecting complex aerodynamic effects hinders high-speed yet high-precision multirotor autonomy. In this paper, we present a computationally efficient learning-based model predictive controller that simultaneously optimizes a trajectory that can be tracked within the physical limits (on thrust and orientation) of the multirotor system despite unknown aerodynamic forces and adapts the control input. To do this, we leverage the well-known differential flatness property of multirotors, which allows us to transform their nonlinear dynamics into a linear model. The main limitation of current flatness-based planning and control approaches is that they often neglect dynamic feasibility. This is because these constraints are nonlinear as a result of the mapping between the input, i.e., multirotor thrust, and the flat state. In our approach, we learn a novel representation of the drag forces by learning the mapping from the flat state to the multirotor thrust vector (in a world frame) as a Gaussian Process (GP). Our proposed approach leverages the properties of GPs to develop a convex optimal controller that can be iteratively solved as a second-order cone program (SOCP). In simulation experiments, our proposed approach outperforms related model predictive controllers that do not account for aerodynamic effects on trajectory feasibility, leading to a reduction of up to 55% in absolute tracking error.

==> experimentalvalidation.tex <==
\section{EXPERIMENTAL VALIDATION}
- Landing and ground effect 
- Flying close to a wall 
- Fan for wind disturbance — fancier contraption to vary intensity of wind

==> methodology2.tex <==


\section{METHODOLOGY}
\{Learning force disturbance as independent GPs Assume Fd(z) We present an algorithm to solve the optimal control problem as an SOCP (ensuring thrust feasibility with high probability) with three key components:\}
 \begin{enumerate}
     \item Probabilistic constraint tightening of thrust constraints
     \item Linearization of GP (LinGP)
     \item Learning-Based MPC as SOCP
 \end{enumerate}
 Since we are unable to establish bounds on the disturbances, we must handle unbounded disturbances with a known probability distribution. To address this, we incorporate a chance constraint into our optimization problem, effectively transforming the MPC into a stochastic MPC problem.
\subsection{Model predictive control (MPC)}
We formulate the path planning problem as an online convex optimization problem where the objective is to follow a reference trajectory while ensuring dynamic feasibility. The optimization problem is subject to a few constraints such as initial state, linear flat dynamics, and two second order cone sets to ensure that the cost function remains linear. To guarantee the feasibility of the control input, we enforce two additional constraints on thrust. Since, there are unknown unbounded disturbances acting on the vehicle we can not guarantee that thrust remains in the these sets all the time. Therefore, we introduce these constraints as probabilistic chance constraints.
\begin{equation}
\begin{aligned}
    &\underset{\mathbf{z},\mathbf{v},q_z,q_v}{\text{min}}
    \sum_{i=0}^{N-1} (q_{z(i)} +q_{v(i)}) + q_{z(N)}\\
    &\textrm{s.t.}\\
    &\mathbf{z}_{0}= \mathbf{z}_{\text{init}}\\
    &\mathbf{z}_{i+1} = \mathbf{F}\mathbf{z}_i + \mathbf{G}\mathbf{v}_i\\
    &(\mathbf{z}_i-\mathbf{z}_{r(i)})^T\mathbf{Q}(\mathbf{z}_i-\mathbf{z}_{r(i)}) \leq q_{z(i)}\\ 
    &\mathbf{v}_i^T\mathbf{R}\mathbf{v}_i \leq q_{v(i)}\\
    &Pr(\mathbf{T} \in S_{\text{cone}}) \geq p_c\\
    &Pr(\mathbf{T} \in S_{\text{ball}}) \geq p_b\\
    &\text{where}
    \quad \mathbf{z} = \begin{bmatrix}
    \textit{\textbf{p}}\\
    \textit{\textbf{v}}\\
    \textit{\textbf{a}}\\
    \textit{\textbf{j}}\\
    \psi
    \end{bmatrix}, \quad \mathbf{v} = \begin{bmatrix}
    \textit{\textbf{s}}\\
    \dot{\psi}
    \end{bmatrix}, \quad \mathbf{y} = \begin{bmatrix}
    \textit{\textbf{p}}\\
    \psi
    \end{bmatrix}
\end{aligned}
\end{equation}

Where $\mathbf{z}\in \mathbb{R} ^ n$ is the vector of flat states consisting of position, velocity, acceleration, jerk, and yaw, $\mathbf{v} \in \mathbb{R} ^ m $ is the vector of flat inputs including snap, and yaw rate, and $\mathbf{y} \in \mathbb{R} ^ l$ is the vector containing the flat outputs which is composed of position and yaw. $\mathbf{z}_r \in \mathbb{R} ^ n$ is the vector of reference states. $q_z \in \mathbb{R}$ and $q_v \in \mathbb{R}$ are dummy optimization variables that are added to ensure the cost function remains linear. Refer to \cite{c4} for more information. $\mathbf{F} \in \mathbb{R}^{n \times n}$, $\mathbf{G} \in \mathbb{R}^{n \times m}$ are the discrete representation of the system's state space. $\mathbf{Q} \in \mathbb{R}^{n\times n}$ $\mathbf{Q} \succcurlyeq 0$ and $\mathbf{R} \in \mathbb{R}^{m \times m}$ $\mathbf{R} \succ 0$ are the weighting matrices in the cost function. The two constraints \((\mathbf{z}_i-\mathbf{z}_{r(i)})^T\mathbf{Q}(\mathbf{z}_i-\mathbf{z}_{r(i)}) \leq q_{z(i)}\) and \(\mathbf{v}_i^T\mathbf{R}\mathbf{v}_i \leq q_{v(i)}\) can be written in matrix form as:\\
\begin{equation}
\footnotesize
    \begin{aligned}
     &\newcommand{\norm}[1]{\left\lVert#1\right\rVert}\norm{\begin{bmatrix}\sqrt{\mathbf{Q}}  &0\\0&-1\end{bmatrix}\begin{bmatrix}\mathbf{z}_i\\q_{z(i)}\end{bmatrix}+\begin{bmatrix}-\sqrt{\mathbf{Q}}\mathbf{z}_{r(i)}\\1\end{bmatrix}}_2\leq \begin{bmatrix}0& 1\end{bmatrix} \begin{bmatrix}\mathbf{z}_i\\q_{z(i)}\end{bmatrix} + 1\\ \\
    &\newcommand{\norm}[1]{\left\lVert#1\right\rVert}\norm{\begin{bmatrix}\sqrt{\mathbf{R}}  &0\\0& -1\end{bmatrix}\begin{bmatrix}\mathbf{v}_i\\q_{v(i)}\end{bmatrix}+\begin{bmatrix}0\\1\end{bmatrix}}_2\leq \begin{bmatrix}0& 1\end{bmatrix} \begin{bmatrix}\mathbf{v}_i\\q_{v(i)}\end{bmatrix} + 1 \label{eq:numbered_equation}
    \end{aligned}
\end{equation}
\subsection{Linearized Gaussian Processes}
We augment the thrust expression with an additional term to account for disturbances. This term is essentially a Gaussian process with mean function $\mu_d(\mathbf{z})$ and variance $\Sigma_d(\mathbf{z})$.
We are employing the LinGP method \cite{c2} to linearize the Gaussian Process. As stated in (LinGp), linearization is a crucial step. Since, mean and covariance of GPs are nonlinear functions, their computations scale cubically with the size of the dataset. Thus, using the covariance in the cost or constraints makes the optimization non-convex which is computationally demanding. On other hand, linearizing GP using first order Taylor expansion around the previous solution of MPC denoted as $\mathbf{z}^*$ allows us to approximate the mean and covariance as linear and quadratic functions respectively. Since mean and covariance of GP appear in the constraint expressions, having them as linear and quadratic functions helps transform those constraint to SOCs conveniently.     
\{Linearizing the gaussian process used to medel external forces using first order Taylor expansion around $\mathbf{z}^*$ in both $x$ and $z$ axes. Defined a new optimization variable \(\hat{\mathbf{z}}\}\).\\
\begin{equation}
    \begin{aligned}
    &\mathbf{T} = m\mathbf{a} + m\mathbf{g} + \mathbf{F}_d(\mathbf{z}), \quad \mathbf{F}_d(\mathbf{z}) \sim \mathcal{N}(\mu_d,\Sigma_d)\\
    &T_x = ma_x+F_{dx}(\mathbf{z}^*)+\frac{dF_{dx}(\mathbf{z})}{d\mathbf{z}}|_\mathbf{z}^*(\mathbf{z}-\mathbf{z}^*)\\
    &T_z = ma_z+mg+F_{dz}(\mathbf{z}^*)+\frac{dF_{dz}(\mathbf{z})}{d\mathbf{z}}|_\mathbf{z}^*(\mathbf{z}-\mathbf{z}^*)\\
    &F_{d}(\mathbf{z}^*)+\frac{dF_{d}(\mathbf{z})}{d\mathbf{z}}|_\mathbf{z}^*(\mathbf{z}-\mathbf{z}^*) = \begin{bmatrix}
    1\\
    \mathbf{z}-\mathbf{z}^*
    \end{bmatrix}^T
    \begin{bmatrix}
    F_{d}(\mathbf{z}^*)\\
    \frac{dF_{d}(\mathbf{z})}{d\mathbf{z}}|_\mathbf{z}^*
    \end{bmatrix}\\
    = &\hat{\mathbf{z}}^T
    \begin{bmatrix}
    F_{d}(\mathbf{z}^*)\\
    \frac{dF_{d}(\mathbf{z})}{d\mathbf{z}}|_\mathbf{z}^*
    \end{bmatrix}
    \end{aligned}
\end{equation}
Thus, the thrust expression for each axis is a Gaussian distribution which takes the following form:\\
\begin{equation}
    \begin{aligned}
    &T_x \sim \mathcal{N}(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}},\hat{\mathbf{z}}^T\hat{V}^{x}_{\mathbf{z}^{*}}\hat{\mathbf{z}})\\
    &T_z \sim \mathcal{N}(ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}},\hat{\mathbf{z}}^T\hat{V}^{\mathbf{z}}_{\mathbf{z}^{*}}\hat{\mathbf{z}})
    \end{aligned}
\end{equation}
We select squared-exponential (SE) as the kernel function. To compute the posterior mean and variance for each axis, we require 1- $\mathbf{z}$ which is the query point 2- $\mathbf{z}^*$ which is point where the Taylor expansion will be around (previous MPC solution) 3- $X$ (all dataset's inputs), 4- $Y$ (all dataset's output data). \(\hat{m}_{z^{*}}\) has \((n+1) \times 1\) dimension. \(\hat{V}_{z^*}\) has \((n+1)\times(n+1)\) dimension where $n$ is the number of states.
\begin{equation}
    \begin{aligned}
    &k(\mathbf{z}_i,\mathbf{z}_j) = \sigma_{\eta}^2\exp{(-\frac{1}{2}(\mathbf{z}_i-\mathbf{z}_j)^T\mathbf{M}^{-2}(\mathbf{z}_i-\mathbf{z}_j))}+\delta_{ij}\sigma_{\omega}^2\\
    &\hat{m}_{\mathbf{z}^*} = 
    \begin{bmatrix}
    k(\mathbf{z}^*,X)\\
    K^{(1,0)}(\mathbf{z}^*,X)
    \end{bmatrix}
    (K(X,X) + \sigma_n^2I)^{-1}Y\\
    &\hat{V}_{\mathbf{z}^*} =
    \begin{bmatrix}
    k(\mathbf{z}^*,\mathbf{z}^*) & K^{(0,1)}(\mathbf{z}^*,\mathbf{z}^*)\\
    K^{(1,0)}(\mathbf{z}^*,\mathbf{z}^*) & K^{(1,1)}(\mathbf{z}^*,\mathbf{z}^*)\\
    \end{bmatrix}-\\
    &(\begin{bmatrix}
    k(\mathbf{z}^*,X)\\
    K^{(1,0)}(\mathbf{z}^*,X)
    \end{bmatrix} 
    (K(X,X) + \sigma_{\eta}^2I)^{-1}
    \begin{bmatrix} 
    k(X,\mathbf{z}^*)&
    K^{(0,1)}(X,\mathbf{z}^*)
    \end{bmatrix}) \\
    &\text{Where each element of matrices $\hat{m}_{\mathbf{z}^*}$ and $\hat{V}_{\mathbf{z}^*}$ can be written as:}\\
    &k(\mathbf{z}^*,\mathbf{z}^*) = \sigma_{\eta}^{2}\\
    &K^{(0,1)}(\mathbf{z}^*,\mathbf{z}^*) = 0_{1\times n}\\
    &K^{(1,0)}(\mathbf{z}^*,\mathbf{z}^*) = 0_{n\times 1}\\
        &K^{(1,0)}(\mathbf{z}^*,X^{(i)}) = \frac{\partial{k(\mathbf{z},X^{(i)})}}{\partial{\mathbf{z}}}|\mathbf{z}^* \\&= \{\mathbf{M}^{-2}(X^{(i)}-\mathbf{z}^*)k(\mathbf{z}^*,X^{(i)})\}_{n\times 1}\\
    &K^{(0,1)}(X^{(i)},\mathbf{z}^*) = \frac{\partial{k(X^{(i)},\mathbf{z})}}{\partial{\mathbf{z}}}|\mathbf{z}^* \\&= \{(X^{(i)}-\mathbf{z}^*)^T\mathbf{M}^{-2}k(X^{(i)},\mathbf{z}^*)\}   _{1\times n}\\
    &K^{(1,1)}(\mathbf{z}^*,\mathbf{z}^*) = \{\sigma_{\eta}^2\mathbf{M}^{-2}\}_{n\times n}\\ 
    &k(\mathbf{z}^*,X) = 
    \begin{bmatrix}
        k(\mathbf{z}^*,X^{(0)}) & k(\mathbf{z}^*,X^{(1)}) & \cdots & k(\mathbf{z}^*,X^{(K)})
    \end{bmatrix} _{1\times K} \\ 
    &k(X,\mathbf{z}^*) = 
    \begin{bmatrix}
        k(X^{(0)}, \mathbf{z}^*) \\ k(X^{(1)}, \mathbf{z}^*) \\ \vdots \\ k(X^{(K)}, \mathbf{z}^*)
    \end{bmatrix} _{K\times 1} \\ \\
    \end{aligned}
\end{equation}
\subsection{Constraint tightening}
To ensure the feasibility of thrust, we must enforce two types of constraints in our optimization problem:\\ 
1) (Half-space constraint) guarantees that the thrust vector remains in the upper half-space at all times.\\ 
2) (2-Norm Ball constraint) ensures that the magnitude of thrust remains within a certain bound.\\
As mentioned in the previous sections, we formulate these constraints as probabilistic chance constraints due to uncertain disturbances in the thrust expression. To make this stochastic MPC problem tractable in a deterministic way, some additional steps are necessary \cite{c5}.\\
We want to constrain the mean of $\mathbf{T}$ in a tightened set (cone), such that with any level of uncertainty, $\mathbf{T}$ remains in the original cone.\\
\textbf{1) Half-space constraint:}\\
The Half-sapce constraint takes the following form. We should write the constraint in z axis.
\begin{equation}
    \begin{aligned}
    Pr(\mathbf{T} &\in S_{\text{half\_space}}) \geq p_h\\
    \mathbf{T} \in S_{{half\_space}} &= \{\zeta|\; h^T\zeta \leq b\}\\
    \mu_{\mathbf{T}_{z}}\in S_{half\_space} \ominus \Omega &= \{\zeta|\; h^T\zeta \leq b - \Phi^{-1}(p_h)\sqrt{h^T\Sigma^{\mathbf{T}}h}\} \\
    \end{aligned}
\end{equation}
where $\Omega$ is the set containing the uncertainty and $\ominus$ represents the Pontryagin set difference.
\begin{equation}\label{eq:10}
    \begin{aligned}
    &h^T\mu_{\mathbf{T}_{z}} \leq b - \Phi^{-1}(p_h)\sqrt{h^T\Sigma^Th}\\
    &-(ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})\leq-\Phi^{-1}(p_h)\sqrt{\hat{\mathbf{z}}^T\hat{V}_{\mathbf{z}^*}^{z}\hat{\mathbf{z}}}\\
    &\hat{V}_{\mathbf{z}^*}^{z} = L_zL^{T}_z\\
    &-(ma_z + mg + \hat{m}_{\textbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})\leq-\Phi^{-1}(p_h)||L_z^{T}\hat{\mathbf{z}}||_2\\
    &||L_z^{T}\hat{\mathbf{z}}||_2 \leq \frac{1}{\Phi^{-1}(p_h)}(ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}}) 
    \end{aligned}
\end{equation}
Where $\Phi^{-1}(p_h)$ is the quantile function of the gaussian distribution, $h = -1$, and $b = 0$. Cholesky decomposition of $\hat{V}_{\mathbf{z}^*}^{z}$ matrix results in $L_zL^{T}_z$ in which $L_z$ is a lower triangular matrix with real and positive diagonal entries. The half-space inequality constraint in (\ref{eq:10}) is transformed into an SOC constraint. This inequality guarantees that the constraint will be satisfied given the uncertainty in the thrust expression, with probability level $p_h$.\\
\textbf{2) Ball constraint:}\\
The ball constraint takes the following form. We should write the constraint in both $x$ and $z$ axes.
\begin{equation}
    \begin{aligned}
        &Pr(\mathbf{T} \in S_{\text{ball}}) \geq p_b\\
        \mathbf{T} &\in S_{{ball}} = \{\zeta|\;||\zeta||_2 \leq T_{max}\}\\
        \mu_{\mathbf{T}} &\in S_{ball} \ominus \Omega =\\ 
        \{\zeta|\;||\zeta||_2 &\leq T_{max} - \sqrt{\mathcal{X}^2(p_b)\lambda_{max}(\Sigma^\mathbf{T})}\}\\
    \end{aligned}
\end{equation}
Where $T_{max}$ is the maximum possible thrust that the rotors can generate. $\lambda_{max}(\Sigma^{\mathbf{T}})$ represents the maximum eigenvalue of the thrust's covariance matrix.
We assume that covariance of $\mathbf{T}$ is decoupled axis-wise. Therefore, we define the covariance matrix of $\mathbf{T}$ as:
\begin{equation}
    \begin{aligned}
        &cov(\mathbf{T})=\begin{bmatrix}
            cov(T_x) & 0\\
            0 & cov(T_z)
        \end{bmatrix}\\
    \end{aligned}
\end{equation}
As $cov(\textbf{T})$ is a diagonal matrix, $\lambda_{max}$ can be either $cov(T_x)$ or $cov(T_z)$. Since we cannot determine which of them is the maximum eigenvalue, we must consider both of them as our constraints. This approach ensures that the feasible region corresponds to the tighter set.
\begin{equation}
    \begin{aligned}
    &||\mu_{\mathbf{T}}||_2 \leq T_{max} - \sqrt{\mathcal{X}^2(p_b)}\sqrt{cov{(T_x)}}\\
    &||\mu_{\mathbf{T}}||_2 \leq T_{max} - \sqrt{\mathcal{X}^2(p_b)}\sqrt{cov{(T_z)}}\\
     &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}}, ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})||_2\leq\\
    &T_{max} - \sqrt{\mathcal{X}^2(p_b)}\sqrt{\hat{\mathbf{z}}^T\hat{V}_{\mathbf{z}^*}^{x}\hat{\mathbf{z}}}\\
    &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}}, ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})||_2\leq\\
    &T_{max} - \sqrt{\mathcal{X}^2(p_b)}\sqrt{\hat{\mathbf{z}}^T\hat{V}_{\mathbf{z}^*}^{z}\hat{\mathbf{z}}}\\
    &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}}, ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})||_2 +\\ &\sqrt{\mathcal{X}^2(p_b)}||L_{x}^T\hat{\mathbf{z}}||_2\leq T_{max}\\
    &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}}, ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})||_2 +\\ &\sqrt{\mathcal{X}^2(p_b)}||L_{z}^T\hat{\mathbf{z}}||_2\leq T_{max}\\
    \end{aligned}
\end{equation}
Where $\mathcal{X}^2(p_b)$ is the quantile function of the chi-squred distribution.\\
Dummy variables \(f\), \(g_x\), \(g_z\) are added at this line.
\begin{equation}
    \label{eq:16}
    \begin{aligned}
        &\begin{cases}
          f + \sqrt{\mathcal{X}^2(p_b)}g_x \leq T_{max}\\
          ||L_{x}^T\hat{\mathbf{z}}||_2\leq g_x\\
          f + \sqrt{\mathcal{X}^2(p_b)}g_z \leq T_{max}\\
          ||L_{z}^T\hat{\mathbf{z}}||_2\leq g_z\\
          ||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}}, ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}})||_2\leq f
        \end{cases}   
    \end{aligned}
\end{equation}
Equation (\ref{eq:16}), derived from the ball constraints, introduces five supplementary constraints to the optimization problem. Among these, two are linear inequality constraints, while the remaining three take the form of second-order cones.\\
\textbf{3) Icecream cone constraint:} \\
To ensure that the thrust vector remains within a certain angle from the $z$ axis, icecream cone constraint must be enforced. 
\begin{equation}
    \begin{aligned}
    &Pr(\mathbf{T} \in S_{icecream}) \geq p_i\\
    &Pr(||T_x||_2 \leq tan\theta_{max}T_z) \geq p_i\\
    \end{aligned}
\end{equation}
Where $\theta_{max}$ is the maximum possible angle between $z$ axis and the thrust vector. The icecream cone constraint can be divided into a half-space and a ball constraint.
\begin{equation}
    \begin{aligned}
    &\begin{cases}
    Pr(r \leq tan\theta_{max} T_z) \geq p_i\\
    Pr(||T_x||_2\leq r) \geq p_i\\
     \end{cases}\\  
    \end{aligned}
\end{equation}
Dummy variable $r$ is introduced at this line. The half-space constraint takes the following form:
\begin{equation}
    \begin{aligned}
     &Pr(-tan\theta_{max}T_z \leq -r) \geq p_i \\
     &-tan\theta_{max}(ma_z + mg + \hat{m}^{T<z>}_{\mathbf{z}^*}\hat{\mathbf{z}}) \leq -r - \Phi^{-1}(p_i)\\
     &tan\theta_{max}\sqrt{\hat{\mathbf{z}}^T\hat{V}_{\mathbf{z}^*}^{z}\hat{\mathbf{z}}}\\
     &\hat{V}_{\mathbf{z}^*}^{z} = L_zL^{T}_z\\
     &||L_z^{T}\hat{\mathbf{z}}||_2 \leq \frac{tan\theta_{max}(ma_z + mg + \hat{m}_{\mathbf{z}^{*}}^{T \prec z \succ}\hat{\mathbf{z}}) - r}{tan\theta_{max}\Phi^{-1}(p_i)}\\
    \end{aligned}
\end{equation}
Ball constraint takes the following form:
\begin{equation}
    \begin{aligned}
     &||\mu_{Tx}||_2\leq r - \sqrt{\mathcal{X}^2(p_i)} \sqrt{cov(T_x)}\\
     &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}})||_2 \leq r - \sqrt{\mathcal{X}^2(p_i)} \sqrt{cov(T_x)}\\
      &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}})||_2 \leq r - \sqrt{\mathcal{X}^2(p_i)} \sqrt{\hat{\mathbf{z}}^T\hat{V}_{\mathbf{z}^*}^{x}\hat{\mathbf{z}}}\\
      &||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}})||_2 + \sqrt{\mathcal{X}^2(p_i)} ||L_{x}^T\hat{\mathbf{z}}||_2 \leq r\\
    \end{aligned}
\end{equation}
Where $\mathcal{X}^2(p_i)$ is the quantile function of the chi-squred distribution.
A procedure similar to that in (\ref{eq:16}) is employed here, leading to the introduction of three additional constraints to the optimization problem.
\begin{equation}
    \begin{aligned}
        &\begin{cases}
          h + \sqrt{\mathcal{X}^2(p_i)}g_c \leq r\\
          ||L_{x}^T\hat{\mathbf{z}}||_2\leq g_c\\
          ||(ma_x + \hat{m}_{\mathbf{z}^{*}}^{T \prec x \succ}\hat{\mathbf{z}})||_2\leq h
        \end{cases}   
    \end{aligned}
\end{equation}
